Young asteroid families as the primary source of meteorites

Understanding the origin of bright shooting stars and their meteorite samples is among the most ancient astronomy-related questions that at larger scales has human consequences [1-3]. As of today, only ${\sim}\,6\%$ of meteorite falls have been firmly linked to their sources (Moon, Mars, and asteroid (4) Vesta [4-6]). Here, we show that ${\sim}\,70\%$ of meteorites originate from three recent breakups of $D > 30\,{\rm km}$ asteroids that occurred 5.8, 7.5 and less than ${\sim}\,40$ million years ago. These breakups, including the well-known Karin family [7], took place in the prominent yet old Koronis and Massalia families and are at the origin of the dominance of H and L ordinary chondrites among meteorite falls. These young families distinguish themselves amidst all main belt asteroids by having a uniquely high abundance of small fragments. Their size-frequency distribution remains steep for a few tens of millions of years, exceeding temporarily the production of metre-sized fragments by the largest old asteroid families (e.g., Flora, Vesta). Supporting evidence includes the existence of associated dust bands [8-10], the cosmic-ray exposure ages of H-chondrite meteorites [11,12], or the distribution of pre-atmospheric orbits of meteorites [13-15].

==> abstract.tex <==

Understanding the origin of bright shooting stars and their meteorite samples
is among the most ancient astronomy-related questions
that at larger scales has human consequences
\cite{Chladni_1794,Biot_1803AnP....15...74B,Kulik_1922}.
As of today, only ${\sim}\,6\%$ of meteorite falls have been firmly linked to their sources
(Moon, Mars, and asteroid (4) Vesta;
\cite{Marvin_1983GeoRL..10..775M,Treiman_2000P&SS...48.1213T,Thomas_1997Sci...277.1492T}).
Here, we show that ${\sim}\,70\%$ of meteorites originate
from three recent breakups of $D > 30\,{\rm km}$ asteroids
that occurred 5.8, 7.5 and less than ${\sim}\,40$ million years ago.
These breakups,
including the well-known Karin family \cite{Nesvorny_2002Natur.417..720N},
took place in the prominent yet old Koronis and Massalia families
and are at the origin of the dominance of H and L ordinary chondrites
among meteorite falls.
These young families distinguish themselves amidst all main belt asteroids
by having a uniquely high abundance of small fragments.
Their size-frequency distribution remains steep for a few tens of millions of years,
exceeding temporarily the production of metre-sized fragments by the largest old asteroid families
(e.g., Flora, Vesta).
Supporting evidence includes the existence of associated dust bands
\cite{Sykes_1990Icar...85..267S,Reach_1997Icar..127..461R,Nesvorny_2003ApJ...591..486N},
the cosmic-ray exposure ages of H-chondrite meteorites
\cite{Graf_1995JGR...10021247G,Eugster_2006mess.book..829E},
or the distribution of pre-atmospheric orbits of meteorites
\cite{Spurny_2020M&PS...55..376S,Brown_2016Icar..266...96B,Jenniskens_2016Icar..266..384J}.


